Password Strength Signaling: A Counter-Intuitive Defense Against Password Cracking

We introduce password strength information signaling as a novel, yet counter-intuitive, defense mechanism against password cracking attacks. Recent breaches have exposed billions of user passwords to the dangerous threat of offline password cracking attacks. An offline attacker can quickly check millions (or sometimes billions/trillions) of password guesses by comparing their hash value with the stolen hash from a breached authentication server. The attacker is limited only by the resources he is willing to invest. Our key idea is to have the authentication server store a (noisy) signal about the strength of each user password for an offline attacker to find. Surprisingly, we show that the noise distribution for the signal can often be tuned so that a rational (profit-maximizing) attacker will crack fewer passwords. The signaling scheme exploits the fact that password cracking is not a zero-sum game i.e., the attacker's profit is given by the value of the cracked passwords minus the total guessing cost. Thus, a well-defined signaling strategy will encourage the attacker to reduce his guessing costs by cracking fewer passwords. We use an evolutionary algorithm to compute the optimal signaling scheme for the defender. As a proof-of-concept, we evaluate our mechanism on several password datasets and show that it can reduce the total number of cracked passwords by up to $12\%$ (resp. $5\%$) of all users in defending against offline (resp. online) attacks.

==> sections/example/theoretical_example.tex <==
%!TEX root=../main.tex
Having presented our Stackelberg Game model for information signaling we now give an (admittedly contrived) example of a password distribution where information signaling can dramatically reduce the percentage of cracked passwords. We assume that the attacker has value $v = 2k + \epsilon$ for each cracked password where the cost of each password guess is $k$ and $\epsilon>0$ is a small constant.

\paragraph{Password Distribution} Suppose that $\mathbb{P}=\{\text{pw}_i\}_{i \geq 1}$ and that each password $pw_i$ has probability $2^{-i}$ i.e., $\Pr\limits_{pw \sim \mathcal{P}}\left[pw= i\right] = 2^{-i}$. The weakest password $pw_1$ would be selected with probability $1/2$. 

\paragraph{Optimal Attacker Strategy without Signaling}
% By checking the top $B$ passwords in descending order of probability (the checking sequence is $\pi$) the adversary has an expected cost of:
% \begin{align*}
% C(k,\pi,B) &= k\sum_{i=1}^{B} i \times 2^{-i} + 2^{-B} \times B \times k = k(2-2^{1-B}),
% \end{align*}
% and an expected reward of
% $$
% R(v,k,\pi,B) = v \sum_{i=1}^{B} 2^{-i} = v \left(1-2^{-B}\right) \ ,
% $$
% which leads to expected profits of 
From equation \eqref{eq:utility}, by checking the top $B$ passwords in descending order of probability the attacker's utility is
$$U_{adv}(v,k,\pi,B) = (v-2k) + (2k-v)2^{-B}.$$

A profit-motivated adversary is interested in calculating $B^* = \underset{B}{\text{argmax }} U_{adv}(v,k,\pi,B)$. With our example distribution we have
\[
B^* = 
\begin{cases}
0 & \mbox{if } v \leq 2k,\\
\infty & \mbox{if } v > 2k.
\end{cases}
\]

Since we assume that $v = 2k + \epsilon > 2k$ the attackers optimal strategy is $B^* = \infty$ meaning that $100\%$ of passwords will be cracked.

\paragraph{Signaling Strategy}
Suppose that $\mathsf{getStrength}$ is define such that $\mathsf{getStrength}(pw_1)=0$ and $\mathsf{getStrength}(pw_i)=1$ for each $i > 1$. Intuively, a the strength level is $0$ if and only if we sampled the weakest password from the distribution. Now suppose that we select our signaling matrix  $$\mathbf{S} = \begin{bmatrix}
1/2 & 1/2 \\
0 & 1 
\end{bmatrix}\ ,$$
such that $\Pr[Sig = 0 ~|~ pw = pw_1] = \frac{1}{2} = \Pr[Sig = 1 ~|~ pw = pw_1]$ and $\Pr[Sig = 1 ~|~ pw \neq pw_1] = 1$. 

\paragraph{Optimal Attacker Strategy with Information Signaling}
We now analyze the behavior of a rational attacker under signaling when given this signal matrix and password distribution.  Again password value is $v = 2k + \epsilon$. 

If the attacker observes the signal $Sig = 0$ we know for sure that the user selected the most common password as $\Pr[pw = pw_1 ~|~ Sig = 0] = 1$ so as long as $v \geq k$ the attacker will crack the password. 

We now consider the case that the attacker facing $Sig = 1$. We have the following posterior probabilities for each of the passwords in the distribution:
\begin{align*}
\Pr[pw = pw_1 ~|~ Sig = 1] %&= \frac{\Pr[s = 1 ~|~ pw = pw_1]\Pr[pw = pw_1]}{\Pr[sig = 1]}\\
&= \frac{0.5*0.5}{0.75} = \frac{1}{3},\\
\Pr[pw = pw_i, i > 1 ~|~ Sig = 1] %&= \frac{\Pr[s = 1~|~ pw = pw_i]\Pr[pw = pw_i]}{\Pr[sig = 1]}\\
&= \frac{1 * 2^{-i}}{0.75} = \frac{4*2^{-i}}{3}.
\end{align*}

% Now we compute the attacker's expected costs conditioned on $Sig = 1$.
% \begin{equation*}
% \begin{aligned}
% C(k,\pi,B;\mathbf{S},1) &= k\left(\frac{1}{3} + \frac{4}{3}\sum_{i=2}^{B} i*2^{-i}\right)+kB\left(1-\frac{1}{3}-\frac{4}{3}\left(\sum_{i=2}^{B}2^{-i}\right)\right) =k\left(\frac{7}{3} - \frac{2^{3-B}}{3}\right),
% \end{aligned}
% \end{equation*}
% when $B > 0$, with $C(k,\pi,0;\mathbf{S},1) = 0$. For expected reward we have:
% \begin{equation*}
% \begin{aligned}
% R(v,k,\pi,B;\mathbf{S},1) &= v\left(\frac{1}{3} + \frac{4}{3}\sum_{i=2}^B 2^{-i}\right) = v\left(1 - \frac{2^{2-B}}{3}\right),
% \end{aligned}
% \end{equation*}
% where $R(v,k,0;\mathbf{S},1) = 0$ in the case where no guesses are made. Thus, the attacker's profit is given by:
% \begin{equation*}
% \begin{aligned}
% &U_{adv}(v,k,\pi,B;\mathbf{S},1) \\
% &= R(v,k,\pi,B;\mathbf{S},1) - C(k,\pi,B;\mathbf{S},1) \\
% &= v\left(1 - \frac{2^{2-B}}{3}\right) - k\left(\frac{7}{3} - \frac{2^{3-B}}{3}\right).
% \end{aligned}
% \end{equation*}
Plugging in $v = 2k+\epsilon$ and posterior probabilities to equation \eqref{eq:uadvsig} we have
% \begin{equation*}
% \begin{aligned}
% C(k,\pi,B;\mathbf{S},1) 
%  &=k\left(\frac{7}{3} - \frac{2^{3-B}}{3}\right),
% \end{aligned}
% \end{equation*}
% when $B > 0$, with $C(k,\pi,0;\mathbf{S},1) = 0$. For expected reward we have:
% \begin{equation*}
% \begin{aligned}
% R(v,k,\pi,B;\mathbf{S},1) &= v\left(\frac{1}{3} + \frac{4}{3}\sum_{i=2}^B 2^{-i}\right) = v\left(1 - \frac{2^{2-B}}{3}\right),
% \end{aligned}
% \end{equation*}
% where $R(v,k,0;\mathbf{S},1) = 0$ in the case where no guesses are made. Thus, the attacker's profit is given by:
% \begin{equation*}
% \begin{aligned}
% &U_{adv}(v,k,\pi,B;\mathbf{S},1) 
% &= v\left(1 - \frac{2^{2-B}}{3}\right) - k\left(\frac{7}{3} - \frac{2^{3-B}}{3}\right).
% \end{aligned}
% \end{equation*}
% Plugging in $v = 2k+\epsilon$ we have
\begin{equation*}
\begin{aligned}
U_{adv}(2k + \epsilon,k,\pi,B;\mathbf{S},1) = -\frac{1}{3}k + \epsilon\left(1-\frac{2^{2-B}}{3}\right) \ .
\end{aligned}
\end{equation*}
Assuming that $\epsilon < \frac{1}{3}k$ the attacker will have negative utility $U_{adv}(2k + \epsilon,k,\pi,B;\mathbf{S},1) < 0$ whenever $B>1$\footnote{If instead we had fixed $v = 4k$ instead we would have $U_{adv}(4k,k,\pi,B;\mathbf{S},1)= k\left(\frac{5}{3} - \frac{2^{3-B}}{3}\right)$ which is maximized at $B^* = \infty$.}. Thus, when the signal is $Sig=1$ the optimal attacker strategy is to select $B^* = 0$ (i.e., don't attack) to ensure zero utility. In particular, the attacker cracks the password if and only if $Sig=0$ which happens with probability $1-\Pr[Sig=1]=0.25$ since $\Pr[Sig=1] =$ $\Pr[pw=pw_1]\Pr[Sig=1 ~|~ pw = pw_1] + \Pr[pw \neq pw_1]\Pr[Sig=1 ~|~ pw \neq pw_1] $ $= \frac{3}{4} $. Thus, the attacker will only crack $25\%$ of passwords. 


\paragraph{Discussion} In our example an attacker with value $v = 2k + \epsilon$ cracks $100\%$ of passwords when we don't use information signaling. However, if our information signaling mechanism (above) were deployed, the attacker will only crack $25\%$ of passwords --- a reduction of $75\%$! Given this (contrived) example it is natural to ask whether or not information signaling produces similar results for more realistic password distributions. We explore this question in the next sections.



==> sections/introold.tex <==

The quest to replace passwords have never ceased (biometrics, graphics, tokens, etc.), but no alternative has been found to retain all the benefits in usability, deployability and security that textual passwords already provide~\cite{SP:Bonneau12}. Therefore, despite of notorious security problems, textual passwords remain the dominant end-user authentication method. Current password storage procedures consist of password hashing, salting and adding pepper. The rational behind these procedures is to further increase the cost asymmetry of checking passwords for the server and the attacker. We would like to explore another direction of decreasing the information asymmetry between the server and the adversary. 

Often the objective of an attacker is to extract as much monetary rewards as possible from password cracking while the defender prioritize minimizing the percentage of cracked passwords in case an offline attack occurs. Their goals appear to be competing and irreconcilable. However, this is not a strict zero-sum game, one party’s loss does not imply the other party’s gain. For example, consider an attacker who purchased or rented super expensive state-level resources which enable the attacker to breach all users’ account of some company, but the costs far exceed rewards. Both parties lose In this example. A natural question would be is there a scenario where both parties win. We resort to information signaling to address this question. Concept of signaling was first brought up in the literature of economics as an approach of narrowing down informational gap. To see why decreasing information asymmetry might benefit both parties, consider another extreme example. Suppose all passwords that a company stores are strong in the sense of guessability, eg., require at least $10^{10}$ dictionary checks to break one,  and monetary reward is going to be far less than the investing cost. The company announces this piece of information and the attacker knows that the company is playing with total honesty. Instead of wasting prohibitive amount of  money in cracking a tough nut that does not worth much,  the best strategy for the attacker would be just giving up. In this case, everyone is better off with information of password strength being signaled. 

All passwords stored are strong in the second extreme example, signaling all passwords strength essentially publishes a credible threat, deterring the adversary from trying to crack passwords. This ideal case does not hold true in reality.  If the server is still totally honest and outputs true signals (denoting password strength with probability 1), then all strength information will be revealed and it will facilitate the attacker to filter the checking list. if the revealed strength is ``weak’’, then the adversary would not even bother to try strong candidate passwords in the checking list. Total honesty for a dataset with heterogeneous strength passwords would expedites the cracking process, which defeats our purpose. Therefore, we argue that the server should play mixed strategy, only partially reveal the strength information. How the mixed strategy is specified is the focus of this paper. 
\subsection{Contributions}
Our contributions are threefold.
\begin{itemize}
\item We propose password signaling, a password storage scheme, to defend against offline/online attacks without altering underlying hash algorithm.
\item We model the interaction between the authentication and the adversary using a classic Stackelberg game, and find the mixed strategy Subgame Perfect Equilibrium (PBE) using an evolutionary algorithm. 
\item We test password signaling with three large empirical datasets, RockYou, Yahoo and LinkedIn. Empirical experiments shows that at PBE,  partially revealing strength information will result in less passwords being cracked than the case all strength information is hidden. Reduction of cracked passwords for Linkedin is up to 13\% when password distribution is known to the server (signaling with perfect knowledge) and 8\% when password distribution is unknown to the server (signaling with imperfect knowledge).
\end{itemize}

\subsection{Related Work}

\subsubsection{Stored Password Records}

The addition of ``salt'' is a crucial defense against rainbow table attacks~\cite{C:Oechslin03} i.e., instead of storing $(u, H(pwd_u))$ and authentication server will store $(u,s_u,H(s_u,pwd_u))$ where $s_u$ is a random string called the salt value. Salting defends against pre-computation attacks (e.g.,~\cite{EC:DodGuoKat17}) and ensures that each password hash will need to be cracked independently e.g., even if two users $u$ and $u'$  select the same password we will have $H(s_{u'},pwd_{u'}) \neq H(s_u,pwd_u)$ with high probability as long as $s_u \neq s_{u'}$.  

Manber proposed the additional inclusion of a short random string called ``pepper'' which would not be stored on the server~\cite{manber1996simple} e.g., instead of storing  $(u,s_u,H(s_u,pwd_u))$ the authentication server would store $(u,s_u,H(s_u,x_u,pwd_u))$ where the pepper $x_u$ is a short random string that, unlike the salt value $s_u$, is not recorded. When the user authenticates with password guess $pwd'$ the server would evaluate $H(s_u,x,pwd')$ for each possible value of $x \leq x_{max}$ and accept if and only if $H(s_u,x,pwd') = H(s_u,x_u,pwd_u)$ for some value of $x$. The potential advantage of this approach is that the authentication  server can usually halt early when the legitimate user authenticates, while the attacker will have to check every different value of $x\in [1,x_{max}]$ before rejecting an incorrect password. Thus, on average the attacker will need to do more work than the honest server. 

Blocki and Datta observed that non-uniform distributions over the secret pepper value $x \in [1,x_{max}]$ can sometime further increase the attacker's workload relative to an honest authentication server~\cite{BlockiD16}. They showed how to optimally tune the pepper distribution by using  stackelberg game theory. Besides considering to tip the scale of hash cost at the server side, Blocki also explored cost asymmetry at client side \cite{DBLP:BlockiS16}. Client-CASH randomizes the runtime of the client-side key stretching so that on average, so that the cost of verifying a correct password is smaller than the cost of rejecting an incorrect password.

\subsubsection{Information Signaling} 

Signaling theory was initially developed by Michael Spence in job market model \cite{10.2307/1882010}. The knowledge of ability of prospective employees are known to themselves but not to the employer. Employees send a signal about their ability level to the employer by acquiring education credentials. The informational value of the credential comes from the fact that the employer believes the credential is positively correlated with having the greater ability and difficulty for low ability employees to obtain. Thus the credential enables the employer to reliably distinguish low ability workers from high ability workers.

\subsubsection{Improving Password Strength} Encouraging (or forcing ) users to select stronger passwords during account creation \cite{campbell2011impact,Komanduri2011,Shay2010,Stanton2005,Inglesant2010,Shay2014} is also a way of defense against offline attacks.  Strict password composition policies (e.g., requiring user's to select passwords that contain numbers and/or capital letters) inevitably introduce a high usability cost \cite{Inglesant2010,NIST2014,Florencio2014lisa,Adams1999} while the strength of passwords generated with such help does not increase significantly\cite{campbell2011impact,Komanduri2011,Shay2010,Stanton2005,Shay2014,Shay2016} --- sometimes stricter policies even result in weaker passwords e.g.,~\cite{blockiPasswordComposition,Komanduri2011}. Password strength meters provide users with dynamic feedback during password creation~\cite{USENIX:KSCHS14,USENIX:UKKLMMPSVBCC12,de2014very}, but the feedback provided by password strength meters is often inaccurate e.g., see~\cite{CCS:GolDur18}. Another line of work focuses on training users to pick stronger passwords e.g., using mnemonic techniques~\cite{Yan2000,AC:BloBluDat13,NDSS:BKCD15,CCS:YLCXP16} and/or spaced repetition~\cite{AC:BloBluDat13,NDSS:BKCD15,blum2015publishable,USENIX:BonSch14}. 

 % Another extensive line of research explored the use of password composition policies in which legitimate password must meet certain requirements, for example, contain numbers and/or capital letters~\cite{campbell2011impact,blockiPasswordComposition,Komanduri2011,Shay2010,Stanton2005,Shay2014,Shay2016}. Empirical studies suggest that strict password requirements inevitably introduce a high usability cost for users~\cite{Inglesant2010,NIST2014,Florencio2014lisa,Adams1999}, while the strength of passwords generated with such help does not increase significantly\cite{campbell2011impact,Komanduri2011,Shay2010,Stanton2005,Shay2014,Shay2016}.  In fact, sometimes stricter policies can result in weaker passwords e.g.,~\cite{Komanduri2011}.

%In fact, sometimes things might go athwart, either resulting in weaker user passwords~\cite{,} or providing inconsistent feedback~\cite{USENIX:UKKLMMPSVBCC12,de2014very}.

%\subsection{Password Cracking and Irreplaceability}
 % Allodi \cite{russianBlackMarket} has studied the economics of the black market for certain attacks and malware, revealing how a password cracking market functions.




%A line of research has focused on encouraging (or forcing ) users to select stronger passwords during the creation process of personal accounts \cite{campbell2011impact,Komanduri2011,Shay2010,Stanton2005,Inglesant2010,Shay2014}. Often instantaneous feedback about strength of current password is given ~\cite{Komanduri2014,USENIX:UKKLMMPSVBCC12,de2014very} or clear instructions towards selection of stronger passwords are provided~\cite{Yan2000,BlockiKCD15}.





%Blocki et al.~\cite{SP:BloHarZho18} developed an economic model to analyze recent password breaches. Under that model quantitative predictions were made about the fraction of accounts that a rational password attacker would crack in case an authentication server breach occurs. The analysis indicates key-stretching levels adopted by PBKDF2 fail to provide sufficient protection for user passwords. However, If memory hard functions were used in password hashing standards, a rational attacker would be deterred from cracking most user passwords
%because MHFs substantially increase guessing costs.

\subsubsection{Memory Hard Functions} Due to the recently complete password hashing competition (PHC~\cite{EPRINT:Wetzels16}) there has been a lot of work on developing secure memory hard functions. There are two types of MHFs: data-independent (iMHFs) and data-dependent (dMHFs). iMHFs are naturally resistant to side channel attacks such as cache timing~\cite{Ber05,AC:ForLucWen14}, but many iMHF constructions are vulnerable to the parallel pebbling attacks of Alwen and Blocki~\cite{C:AlwBlo16,AB17} including PHC winner Argon2i~\cite{Argon2,TCC:BloZho17}, thus reduce the amortized AT complexity of the iMHF. The designers of Argon2~\cite{Argon2} currently recommend running in {\em hybrid mode} Argon2id to balance side-channel resistance and resistance to parallel pebbling attacks on Argon2i.   \cite{EC:AlwBloPie17,CCS:AlwBloHar17} propose DRSample algorithm to bring  the constructive applications of depth-robust and high amortized AT complexity graphs into practice, resulting in nearly-ideal iMHFs that achieve AT complexity $\Omega(t^2/\log t)$. \cite{ABZ20} introduces computationally data-independent memory hard functions (ciMHFs). The memory access pattern induced by the (randomized) ciMHF evaluation algorithm appears to be independent from the standpoint of a computationally bounded eavesdropping attacker, thus resist side-channel attacks while having high cumulative memory complexity.

%The standard signaling game is called Beer-Quiche game. In this game, player 2 is considering whether to duel with another player 1. Player 2 knows that player 1 is either a wimp or is surly but not which. Player 2 would prefer a duel if player 1 is a wimp but not if player 1 is surly. player 1, regardless of type, wants to avoid a duel. Before making the decision player 2 has the opportunity to see whether player 1 chooses to have beer or quiche for breakfast. Both players know that wimps prefer quiche while surlies prefer beer. Separating equilibrium and polling equilibrium are studied by In-Koo Cho and David M. Kreps \cite{QE:Kerps1987}.

==> sections/strategy.tex <==
\subsection{Signaling Strategy}
A signaling matrix of dimension $d$ is determined by $d(d-1)$ variables since the elements in each row sum up to 1. Define $f:\mathbb{R}^{d(d-1)}\rightarrow 
\mathbb{R}$ be the map from $S$ to $P_{ADV}^{wi}$. When password value/hash cost ratio and partition method are fixed, then the optimization problem becomes
\begin{mini}|s|
{\mathbf S}{ f (s_{11},\ldots s_{1(d-1)}, \ldots, s_{d1},s_{d(d-1)})}
{}{}
\addConstraint{0 \leq s_{ij} \leq 1, \; \forall 1\leq i\leq d,\; 1\leq j\leq d-1}
\addConstraint{\sum_{j=1}^{d-1} s_{ij} \leq 1,\; \forall 1\leq i\leq d}.
\end{mini}
The feasible region is a $d$-dimension probability simplex. (Notice that in 2-D, the second constraint would be equivalent to the first constraint.) Since the underlying function $f$ to be optimized does not assume any specific form,  
it can be treated as a black box that answers function value at a given query point, thus we solve it using global derivative-free optimization methods. Derivative-free optimization is active research area with many mature solvers with simple interface, e.g., CMA-ES, NOMAD, DAKOTA. In our experiment we choose BITmask Evolution OPTimization (BITEOPT) algorithm to compute the quasi-optimal signaling matrix $\mathsf{S}$. 

BITEOPT is a free open-source stochastic non-linear bound-constrained derivative-free optimization method (heuristic or strategy). BiteOpt took 2nd place (1st by sum of ranks) in BBComp2018-1OBJ-expensive competition track. 

BITEOPT maintains a population list of previously evaluated solutions that are ordered in cost (objective function value). The whole population evolves towards a lower cost. On every iteration, the solution with highest cost in the list can be replaced with a new solution, and the list is reordered.  The solution vectors are spanned apart from each other to cover a larger parameter search space collectively. Beside that, a range of parameter randomization and the "step in the right direction" (Differential Evolution "mutation") operations are used that probabilistically make the population evolve to be ``fittest’’ ones (lower cost solutions). BITEOPT’s hyper-parameters (probabilities) were pre-selected and are not supposed to be changed. We give a more detailed introduction of BITEOPT in the appendix.

 

